RefEgo: Referring Expression Comprehension Dataset from First-Person Perception of Ego4D

Grounding textual expressions on scene objects from first-person views is a truly demanding capability in developing agents that are aware of their surroundings and behave following intuitive text instructions. Such capability is of necessity for glass-devices or autonomous robots to localize referred objects in the real-world. In the conventional referring expression comprehension tasks of images, however, datasets are mostly constructed based on the web-crawled data and don't reflect diverse real-world structures on the task of grounding textual expressions in diverse objects in the real world. Recently, a massive-scale egocentric video dataset of Ego4D was proposed. Ego4D covers around the world diverse real-world scenes including numerous indoor and outdoor situations such as shopping, cooking, walking, talking, manufacturing, etc. Based on egocentric videos of Ego4D, we constructed a broad coverage of the video-based referring expression comprehension dataset: RefEgo. Our dataset includes more than 12k video clips and 41 hours for video-based referring expression comprehension annotation. In experiments, we combine the state-of-the-art 2D referring expression comprehension models with the object tracking algorithm, achieving the video-wise referred object tracking even in difficult conditions: the referred object becomes out-of-frame in the middle of the video or multiple similar objects are presented in the video. Codes are available at https://github.com/shuheikurita/RefEgo

==> sec/buffer.tex <==
\begin{comment}
We conduct further analyses on the top-1 bounding box confidence and whether the image includes the referred object with the two finetuned MDETR models: MDETR (Conventional) and MDETR (All images).
Figure~\ref{fig:mdetr_results} presents the confidence used for the detection of the no-referred-object images by the two finetuned MDETR models.
Blue and orange colors represents the number of images that include the referred object annotation (blue) and do not include it (orange).
MDETR (All images) has a shallow distribution of the confidence. It has a high ratio for images that do not include the referred object annotation for the confidence score from 0 to 0.2 while it has relatively high ratio for images that include the referred object in the high confidence score zone, such as the confidence score from 0.7 to 0.9. However, this tendency is unclear for the MDETR (Conventional), which has very few cases for low confidence.
\end{comment}


% \textit{Object-class uniqueness} is the label whether there are any other objects of the same class with the referred object or not.
% \textit{Referred object movement} is the label whether the referred object is moving/moved in the video clip or not.


% In both cases the confidence for the referred target object is not the highest in the prediction as the denoted highest confidence bounding box exist in the Frame $T$.
% The tracker-based model in red bounding boxes, however, successfully track the same object from the frame $T-1$ to the frame $T$ in these two examples, irrelevant to the predicted confidence bounding box in the frame $T$.
% although c we could select the bounding box close to ground truth as a prediction.

% In the RefEgo dataset, videos are drawn from Ego4D and they have first-person features captured by the head-mounted cameras.
% This implies that videos often include the rapid motion of the camera resulting, in the blur image frames
% % and missing overlaps from previouds.
% Even if the target referred expression is presented in the candidates, these features make too difficult to track the same object in a clip because an object moves too much and there is no overlap between adjacent frames.
% As a result, the object tracking baseline, MDETR with ByteTrack could not exceed MDETR w/o ByteTrack. 
% Some images are often too blurred. The target object can be out of the frame for some of images in video clips.

% These features make by far difficult to track the same object in a clip compared to the previous object tracking datasets. 




% Figure~\ref{fig:qualitative_analyses} presents the qualitative results for MDETR and OFA models in comparison to annotated bounding box.


\subsection{Object tracking}
\label{sec:object_tracking}

\begin{comment}
inconsistencyを緩和するために， MDETR(all images)の予測に対してTracking手法のSoTAであるByteTrackを適用した．　ByteTrackにおけるパラメータは，high score　detection boxesのthresholdは0.5, low score detection boxesのthresholdは0.1にした． 
隣接フレーム間で，objectness scoreが0.01以上かつIoUが0.05以上の物体に対してmatchingを行なった．
また， ByteTrackに適用する前に， 重なっているbounding boxを削減するためにNMSをIoU　threshold=0.5として適用した．　

選択するBounding Boxは以下の条件で各フレームで1つ選択する．
1.　2frameおよび1frame前でそれぞれ異なるobjectとして選択されており，　それぞれにmatchしたobjectが現在のフレームで現れた場合，scoreの高い方を選択
2. 2frameおよび1frame前で選択されたobjectのどちらか一方にmatchしたobjectが現在のフレームで現れた場合，　そのobjectを選択
3. そのほかの場合，　scoreの最も高いobjectを選択

ByteTrackを適用した結果， 本文Figure~\ref{fig:bytetrack}のように誤りを訂正する場合もあるが， Table~\ref{table:sub_experiments_val}のように，Top1と比べて大きく精度を下げる結果となった．　
しかし， RefEgoのデータセットの特性上，　targetのフレーム間の位置の移動幅が大きく，　また，小さな物体も多いため，　IoUでのmatchingではTrackingがうまく機能しないと分かった．

そこで， MDETRではtokenとbounding boxのcontrastive learningも行われているため，　bounding box内の物体におけるembedding featureを利用して， matching algorithmに適用した． ByteTrackではIoUでmatchingしていたものを，物体の位置を考慮せずに， embedding 同士のcosine similarityが0.98以上の物体を同一とするmatching処理を行なった． これをSimTrackとする．

Table~\ref{table:sub_experiments_val}より，　SimTrackもByteTrackと同様にTop1と比べて精度を下げる結果となった．

% mIoU+TN, mIoU0.5+TN をメインに比較
% confidence score? confidence value? 
\end{comment}





% ~\footnote{We didn't apply ByteTrack for OFA results because OFA is able to predict a single bouunding box for each image. This is not suitable for the tracking-based consistent bounding box selection.}.

% We set thresholds of high and low score detection boxes, hyper-parameters of ByteTrack, to 0.5 and 0.1, respectively. For matching objects between adjacent frames, the candidate objects for matching were restricted to the condition that both confidence score (objectness scores) are greater than 0.01 and IoU is greater than 0.05.
% In addition, we apply NMS to predictions in each frame to reduce overlapped bounding boxes.

% For REC task, we selected one bounding box in frame $T$ from the predicted bounding boxes with the base 2D REC model under the following conditions:

\begin{comment}
In training, MDETR is trained with contrastive learning between token and object embeddings. Therefore, we use cosine similarity between object embeddings instead of IoU overlaps for matching. Objects for which cosine similarity is greater than 0.98 in frames are considered identical. We refer to this algorithm as SimTrack. In Table~\ref{table:sub_tracking_result}, we present both results of ByteTrack and SimTrack.
It somehow increases the performance compared to ByteTrack, although we witnessed the strong performance of 2D-based REC models.
\end{comment}

% \katsura{本文の図参照}
% In some cases, ByteTrack is able to detect outlier bounding boxes such as those in frame $T$ of
% Figure~7
% % Figure~\ref{fig:bytetrack}
% in the main paper. However, the entire performance is not improved as Table~\ref{table:sub_tracking_result} presents.
% In the RefEgo dataset, many referred objects are small and/or in motion significantly.
% %from frame to frame.
% From this property, IoU (overlap)-based matching is defamed, making the tracking of some objects difficult.


==> sup/baseline3d.tex <==
\subsection{Ablation: 3D projection baseline}

We finally examined the 3D projection-based model.
% We can infer camera viewpoints for 2D images in 3D scenes.
If we successfully localize the camera viewpoints for 2D images in 3D scenes, we can localize the referred object in the projected 3D scene.
This is similar to the episodic 3D scene memory of the egocentric memory-based QA applied for object localization in 3D scene~\cite{episodic_mem_qa}.
The entire process is visualized in Figure~\ref{fig:3D_localization}.
Given the inferred bounding boxes from 2D REC models, the 3D projection baseline model localizes the referred object in 3D space and then re-project the referred object point into the 2D images.
Although this approach is quite sensitive to the errors of the inferred camera parameters, this can refine the existing 2D REC model results in some cases.


We use COLMAP~\cite{schoenberger2016sfm} structure-from-motion for the estimation of the camera intrinsic and extrinsic parameters from images\footnote{We assume a conventional assumption as a simple radial lens. All images in the same video clip share the same intrinsic parameters.}.
Then we computed the projection of the bounding box corners into four lines of the 3D space for each image.
For each corner, we derive a single point where lines approximately converge\footnote{We ignore lines that are almost parallel or converge at a point distant from others}. This is the projection of the bounding box corner in 3D space.
Once the corners of the bounding box are projected to 3D space, we conversely project the bounding box from 3D to 2D image space.

This approach, however, is quite sensitive to the errors of the intrinsic and extrinsic parameters and indeed it doesn't work well for many of the video clips in RefEgo.
When the referred object is in motion, this approach does not work at all.
RefEgo often include blurred images that make the COLMAP estimation hard. We use the OFA model, which supplies the most accurate boundary boxes for the
In supplementary material, we supply the example of the 3D projection-based model in Figure~\ref{fig:colmap_tomato} and Figure~\ref{fig:colmap_bath}.
In both figures, we can see that the 3D-projection baseline model can localize the same object even for the images where the 2D REC model predicts similar another box (Figure~\ref{fig:colmap_tomato}) or the entire referred object is not in the image (Figure~\ref{fig:colmap_bath}).
We also provide the changes of the entire performance for reference, although we need to be careful for interpreting this result because some referred objects are clearly not suitable for 3D projection.

% When the COLMAP estimation is relatively accurate, the 3D projection baseline

\begin{figure*}[t]
    \centering
    \includegraphics[width=12cm]{fig/3D_localization.png}
    \caption{The localization of the boundary box in 3D projection space.
    We draw the camera positions of images inferred by COLMAP in black pyramids.
    For each camera-position, we draw four-colored lines for the corners of the predicted bounding box. The four red cubes (left top) are the newly inferred corners of the 3D-projected bounding box in black.
    This is the visualization of the example in Figure~\ref{fig:colmap_tomato}.}
    \label{fig:3D_localization}
\end{figure*}


\begin{figure*}[t]
    \centering
    \includegraphics[width=18cm]{fig/colmap_v516_tomato.pdf}
    \caption{The (selected images of) refinement of the 2D REC model results by 3D projection. Annotated (green), OFA prediction (gray) and 3D projection-based boundary boxes (orange). The referring expression is \textit{``the lower right tomato in tomato packet below the spicy containers''.}}
    \label{fig:colmap_tomato}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=18cm]{fig/colmap_v1531_bath.pdf}
    \caption{The (selected images of) refinement of the 2D REC model results by 3D projection. Annotated (green), OFA prediction (gray) and 3D projection-based boundary boxes (orange). The referring expression is \textit{``The white bath tub inside the bathroom.''}}
    \label{fig:colmap_bath}
\end{figure*}

\begin{table*}[t]
\begin{center}
% 	\scriptsize
\footnotesize\begin{tabular}{llcccccccc}
    \toprule
    && \multicolumn{4}{c}{RefEgo Val}  & \multicolumn{4}{c}{RefEgo Test} \\
     \cmidrule(lr){3-6}\cmidrule(lr){7-10}
Model   &         & mIoU & mIoU@50 & mIoU+TN & mIoU@50+TN   & mIoU & mIoU@50 & mIoU+TN & mIoU@50+TN \\
\midrule
OFA &             & 53.2 & 58.6 & 46.5 & 50.2  & 52.8 & 57.8 & 46.5 & 49.9 \\
OFA & +3D proj.   & 27.5 & 24.2 & 30.5 & 29.3  & 29.3 & 26.7 & 32.0 & 30.9 \\
\midrule
MDETR  &          & 46.8 & 54.1 & 48.7 & 54.1  & 46.0 & 53.1 & 48.3 & 53.7 \\
MDETR & +3D proj. & 31.3 & 28.0 & 32.0 & 31.0  & 26.6 & 24.9 & 23.2 & 21.7 \\
\bottomrule
    \end{tabular}
    \caption{
        The performance of the refinement results of the 2D REC models, OFA and MDETR (all images), with 3D projection.
    }
    \label{table:sub_experiments_val}
\end{center}
\end{table*}


==> sup/mdetr_binary_head.tex <==
\section{Ablation studies}
We further examine additional approaches: MDETR binary image classification head, object tracking baseline and 3D projection baseline.
Not limited to the previous 2D REC approach,  we are driven by the motivation to supply multifaceted baseline approaches with our RefEgo dataset.
\textbf{Such baselines are not for the immediate performance boost but for curving the nature and limitations of the current large-scale video-based referring expression comprehension dataset from various approaches.} These ablation studies would be not only the North Star of later studies in various model construction approaches but also suggestions for comparing and choosing approaches for the real-world deployment of the referring expression comprehension systems.


\subsection{Ablation: MDETR with binary image classification head}

In the main paper, we have seen that the confidence scores (objectness scores) are not discriminative well for determining whether the referred object is in the image or not.
Here we add an additional object query to the existing MDETR (all). This additional object query is combined with a binary head to perform the binary classification trained with the binary cross-entropy loss of whether the object is in the image or not.
% We refer to this model as MDETR (binary head).

Table~\ref{table:sub_mdetr_binary_result} presents the performance of MDETR+BH compared to MDETR (all).
Similar to the 
% Table~\ref{table:experiments_main_val}
Table~4
of the paper, we present REC metrics for images that surely include the referred object: $\mathrm{mIoU}$ and $\mathrm{mIoU@50}$. We also present the combination metrics including the detection task for images that do not include the referred object: $\mathrm{mIoU+TN}$ and $\mathrm{mIoU@50+TN}$.
However, the performance of the binary head in Figure~\ref{fig:sub_mdetr_dist} is more discriminative than those achieved by the confidence score (objectness score) of MDETR (all) in 
% Figure~\ref{fig:mdetr_results}
Figure~6
of the paper. 
Therefore, as seen from Table~\ref{table:sub_auc}, the comparison in AUC suggests that the model with the additional binary head achieves the best performance in the detection of images that do not include the referred object.



\begin{figure}[t]
    % \begin{tabular}{c}
        % \begin{minipage}[t]
            % \centering
            \includegraphics[width=8.2cm]{fig/mdetr_conventional_dist.pdf}
        % \end{minipage} \\
        % \begin{minipage}[t]
            % \centering
            \includegraphics[width=8.2cm]{fig/mdetr_all_images_dist.pdf}
        % \end{minipage} \\
        % \begin{minipage}[t]
            % \centering
            \includegraphics[width=8.2cm]{fig/mdetr_binary_head_dist.pdf}
        % \end{minipage}
        \includegraphics[width=8.2cm]{fig/mdetr_binary_head_dist.pdf}  
    \caption{
    The Comparison of histograms for objectness scores of images predicted by two MDETR models.
    Blue: the number of images that include the referred object, aligned by confidence.
    Orange: those for images that do not include the referred object.
    Blue line: the ratio of images that include the referred object in each 0.1-width bin.

    The histograms for binary classification scores whether the referred object is in images or not predicted by MDETR with the binary head (+BH). 
    Blue: the number of images that include the referred object, aligned by confidence.
    Orange: those for images that do not include the referred object.
    Blue line: the ratio of images that include the referred object in each 0.1-width bin.
    }
    \label{fig:sub_mdetr_dist}
\end{figure}



==> tab/fig_qualitative.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=16cm]{fig/figure_compare2.pdf}
    \caption{Comparison of the predicted bounding box, OFA$^{\ddagger}$ and MDETR$^{\ddagger}$ detected objects.}
    \label{fig:qualitative_analyses}
\end{figure*}


==> tab/fig_wordcloud.tex <==


\begin{figure}[t]
    \centering
    \includegraphics[width=6cm]{fig/detic_labels.pdf}
    \caption{Frequently seen object categories in RefEgo by Detic (LVIS).}
    \label{fig:detic labels wordcloud}
\end{figure}

